Early Validation of High-level Requirements on Cyber-Physical Systems

The overarching, broad topic of my research are advancements in the area of safety-critical, cyber-physical systems (CPS) development with emphasis on validation and verification. The particular focus of my research is the early validation of high-level requirements on CPS. My current approach for tackling this problem is transforming the requirements into Event Calculus and subsequently reasoning about them using ASP solvers such as the grounding-free s(CASP). Below, I discuss my research, its current state, and the open issues that are still left to tackle. The first results of my work will be presented in a paper that was accepted for ICLP'24, which is my first paper in this area.

==> eptcsdata.tex <==
\providecommand{\firstpage}{390}
\providecommand{\publicationstatus}{P. Cabalar, F. Fabiano, M. Gebser, G. Gupta and Th. Swift (Eds.):\\ 40th International Conference on Logic Programming (ICLP 2024)\\
EPTCS 416, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.416.40}{10.4204/EPTCS.416.40}}

